The Impact of Visibility on the Right to Opt-out of Sale under CCPA

The California Consumer Protection Act (CCPA) gives users the right to opt-out of sale of their personal information, but prior work has found that opt-out mechanisms provided under this law result in very low opt-out rates. Privacy signals offer a solution for users who are willing to proactively take steps to enable privacy-enhancing tools, but many users are not aware of their rights under CCPA. We therefore explore an alternative approach to enhancing privacy under CCPA: increasing the visibility of opt-out of sale mechanisms. We conduct an user study with 54 participants and find that visible, standardized banners significantly increase opt-out of sale rates in the wild. Participants also report less difficulty opting out and more satisfaction with opt-out mechanisms compared to the native mechanisms currently provided by websites. Our results suggest that effective privacy regulation depends on imposing clear, enforceable visibility standards, and that CCPA's requirements for opt-out of sale mechanisms fall short.

==> sections/20-related.tex <==
\section{Related Work}

Recent privacy regulations, notably CCPA and GDPR, have given rise to questions about how these regulations impact user privacy and how future regulations might further enhance privacy. This line of work takes place within the context of a larger body of work that has explored user attitutes and beliefs  about data practices and investigated how aspects of user design affect user engagement in general and interactions with privacy mechanisms in particular.

\subsubsection*{User Beliefs about Data Practices}  Privacy regulations are intended to give users increased  control over their personal information. However, prior work has consistently shown that users are generally unaware of how their data is being collected and sold, which websites affect them, and what options they have to control their privacy.  

Machuletz and B\"ohme~\cite{Mach20} showed that around 80\% of users self reported knowledge around cookies, and around 68\% could accurately describe them. Users in the study also generally unaware of the possible consequences of accepting cookies, and demonstrated regret in their choices after interacting with cookie options. 

In a study on behavioral advertising, users were shown to be both generally uneducated about the nature of targeted ads and appalled by an increased knowledge on their function~\cite{Cranor12}. When asked about online behavioral advertising, many users were not aware of its nature or function. When shown a video that explained it to them in more detail, many users felt it was ``scary'' or ``creepy,'' and consistently demonstrated a failure to understand exactly how it worked or what their choices were. To many users, data collection and targeted advertising seem to be ``black boxes." They are aware that these mechanisms exist, but not how they work, how much they see, or what possible recourse they might have. This study suggests that the baseline of user awareness around data collection and its use in targeted advertising is generally poor, suggesting that notices that fail to accurately desribe their purpose or remain hidden on a page are unlikely to be understood or used. 

Habib et al.~\cite{Habib20} conducted long form interviews with users on their data privacy choices and behavior. Users not only demonstrated a similar lack of awareness and education on the topics of cookies and their interactions with privacy mechanisms. The study asked users to interact with services like account deletion, email list opt-outs, and advertising opt-outs on various websites. Users often were unclear about how cookies worked on their different devices, with either misconceptions or a lack of general knowledge about the concept in general. Users showed not only a lack of awareness about these topics and difficulty interacting with these mechanisms, but a general dissolution and distrust that these mechanisms worked at all. To enhance privacy, they recommended standardizing interactions with privacy options. 

\subsubsection*{Usability of CCPA Opt-out Mechanisms}
O'Connor et al.~\cite{oconnor2021clear} investigated the impact of banners versus links on engagement with CCPA opt-out of sale mechanisms. They found that links had significantly lower engagement (and rate of opt-out) than banners, with users just 1.4\% of users opting-out of sale when provided with an opt-out link compared to 12.2\% of users who were shown a banner. They also investigated the effect of banner location, nudging, and inconvenience factors on opt-out rates. The design of banner implemented by COA---which adopts a single-button ``anti-nudging'' design---was informed by their results.  

Cranor et. al. performed a series of studies examining how different taglines and icons influence user comprehension and recall of Do Not Sell links~\cite{cranor2020design,cranor2020user,cranor2020ccpa,cranor2021informing}. They found that most participants failed to notice Do Not Sell links in an image of a website, that users expect links to opt them out in a single click, and that an overwhelming majority of participants were unaware of CCPA and/or misunderstood what kinds of personal information were included in Do Not Sell---all findings that are consistent with our results; they recommended the adoption of standardized icons and placement, along with enforcement of the existing requirement for standardized language for opt-out links. However, their work did not compare the usability of current links or privacy icons with opt-out banners, and it did not consider the impact design choices after the initial opt-out link on usability. 

A Consumer Reports study~\cite{mahoney2020california}, which asked users to attempt to opt-out of sale on 216 websites from the California Data Broker registrar, also studied the usability of opt-out mechanisms adopted by those sites. In their study, three users were asked to attempt to opt-out of sale of their personal data on each site. They found that  31.4\% of the sites studied displayed their link in such a manner that at least one out of three users was unable to find it, that more than a third of participants spent over five minutes opting out (with a maximum time of over an hour), and 14\% ultimately were unable to successfully complete the process. However,  the limited sample size (3 users per website) and the differences in design choices adopted by each site precluded any statistically significant results about the impact of the observed designs on users' awareness of (and likelihood of invoking) their right to opt-out of sale. 

Earlier work also consistently found that opt-out mechanisms were hard for users to understand and use~\cite{habib2020s,habib2019empirical,Leon12,Utz19,sanchez2019can,nouwens2020dark,machuletz2020multiple,sakamoto2019after}. However, those studies were conducted prior to the adoption of CCPA and focused on the usability of opt-out mechanisms under earlier laws, such as the CAN-SPAM Act and GDPR. Nonetheless, the recommendations made by those authors---including requiring specific mechanism positions, increased granularity for privacy choices, and specific text in notices---are likely relevant to CCPA. 


\paragraph*{Tools for Enhacing Privacy under CCPA}
Since enforcement of CCPA began in July 2020, several tools have been release that attempt to enhance privacy under CCPA. Global Privacy Control (GPC)~\cite{GPC} is a standardized privacy signal that asks websites not to sell information about that user; California law now requires websites to respect GPC as a valid mechanism for opt-ing out of sale under CCPA. There are a variety of privacy tools that implement GPC: Firefox, Brave, and the Duck Duck Go mobile browser all offer built-in support for GPC. There are also Chrome extensions (e.g.,  OptMeowt~\cite{Zimmeck20}) that issue GPC signals.  Opt Out~\cite{OptOut}, a Chrome browser extension released by yourdigitalrights.org, sends automatically-formatted opt-out emails to website hosts that invoke a user's rights to Data Access and Data Deletion under GDPR and CCPA, but it does not support requests to opt-out of sale. CCPA Detector~\cite{CCPAdetector} is a Chrome browser extension  that detects CCPA-related privacy policies. However, it us unable to accurately detect which websites sell data, and the effect on end-user privacy has not been experimentally tested. 

Privacy-related browser extensions have also been developed prior to and independent of CCPA; while such tools have the potential to enhance privacy, user studies have found that they are often confusing to users and ineffective. Leon et al.~\cite{Leon12} studied third party extensions, built in browser privacy features, and other cookie blockers. They found that users were confused by the user interface and the description provided,  that users were unclear what the exact purpose of the tools was, and that users were unable to configure the tools to effectively protect their privacy. 

==> sections/50-wild.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/storepage.png}
	\caption{Chrome Web Store page listing for the COA browser extension.}
	\label{fig:store}
\end{figure}




\section{COA in the Wild}\label{section:real-world}


We released COA as a browser extension on the Chrome Web Store in June 2021; a copy of the Chrome Web Store page for the COA browser extension is shown in Figure~\ref{fig:store}. 
%
\subsection{Methodology}

To advertise COA, we  ran an ad campaign on Google Ads between July 1-10, 2021. 
A copy of the ad shown for this campaign is provided in Figure~\ref{fig:adcopy}. Our ad received 245K total impressions and 2095 total clicks, with a cost per click of 36 cents. Users who clicked on the ad were redirected to the  Chrome Web Store page for COA.

\paragraph{Ethical Considerations.} Out of respect for ethical considerations, we minimized what data COA collected. As described in Section~\ref{sec:coa_design}, we did not collect any personally-identifiable information or demographic information. In order to enable us to calculate statistics about how frequently COA users opted-out of sale, we recorded hashes of domains visited; we did not attempt to de-identify these domains and we did not conduct any analysis to infer demographics, interests, or other information about our users. Aside from aggregate statistics reported in this paper, no information about our users was shared with third-parties.

To ensure that users were informed about our data practices, we provided this information---including what data we collected (as described in Section~\ref{sec:coa_design}), how that information would be used, and the fact that COA was released as part of an academic study---in a privacy policy linked from the Chrome Web Store page. Although there was no explicit opt-in within the COA interface, this consent procedure is consistent with both legal standards and cultural norms around data collection in California. 

This user study, including the data collection and consent procedure, was reviewed and approved in advance by the institutional review board at our institution.

%
\subsection{Results}
%
52 unique users installed and used COA for at least 24 hours during that period; due to ethical considerations we did not collect any demographic information about these users. Across these users we logged 1,360 unique websites visited, 37,802 total logs, and 45 opt outs.

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/linkbreakdownreal.png}
%    \caption{How many websites were recorded selling data by real users}
%    \label{fig:realuserlinks}
%\end{figure}

%\subsubsection*{Prevalence of Opt-out Links}

%A significant majority of sites visited by COA users (75.4\%) did not have opt-out of sale links; 24.3\% had valid opt-out links and the remaining four websites (.3\%) had ambiguous links. These results are consistent with the frequency of opt-out links among the Top 5000 websites, but constitute significantly lower rates of sale than users believe (Figure~\ref{fig:sell_rates}). 

\begin{figure}[t!]
    \centering
    \includegraphics[width=.8\columnwidth]{figures/ads-optout_types.png}
    \caption{Opt-out rates among users who downloaded COA from the Chrome extension store.}
    \label{fig:optbreakdown}
\end{figure}


%\subsubsection*{Opt-out Behavior}
In general, users who download COA through the Google Chrome Store opted-out at a higher rate than participants in our MTurk study, likely because these users self-selected by choosing to install an extension relating to CCPA. These users opted out of sale on 18.8\% of sites that provided a link to an opt-out of sale mechanism, on average. a combined total of 45 times. As was the case with participants in the MTurk study, the majority of opt-outs used the button provided in the COA popup banner (53.3\%). An additional 6.7\% of opt-outs were via the button provided in the COA menu; the remaining opt-outs used the native link. %Of these opt outs, 38 were through the extension's popup, 3 were through the extension, and 22 were through a manual interaction with the opt out link. %% these numbers are wrong. corrected now
This distribution reflects slightly higher use of native opt-out links among users in the wild than among participants in our MTurks study---a pattern that might indicate that users who self-select to click on an ad about a privacy extension and install that extension are already more aware of opt-out opportunities than the average user---but the fact that even these users made used COA features more often than native links reinforces our belief that popup banners are an effective method to empower users to interact with opt out mechanisms. 


Encouragingly, users who downloaded COA through the Chrome Web Store continued to opt out of sale of their personal information throughout the time they used the extension. While MTurk users tended to opt out a few times at the beginning of the study and then stop, real-world users continued to opt-out later. Additionally, COA users relied increasingly on banners to access opt-out of sale mechanisms, suggesting that perhaps as COA users became familiar with they extension, they found COA banners to be a convenient, accessible mechanism to opt-out of sale on websites they visit. %The distribution of opt-outs over time is shown in Figure~\ref{fig:optdistribution}. % the number of manual opt outs increased over time, perhaps suggesting that using COA increased awareness about the existance of opt-out mechanisms. % users gain an increased awareness of opt out mechanisms. However, opt outs still were not very frequent. The average user only opted out of 3.3\% of the opt out sites that they visited. Most sites that were opted out only received one or two opt outs across users. Although some top sites received over 10 opt out requests by users, these were the sites that received the most visits, and still were not opted out by many of the users.

These results are consistent with prior work, which has found that active warnings are effective in sparking user action in other contexts~\cite{Egel08}. They suggest that privacy-enhancing tools like COA that provide active warnings may prove effective at enhancing privacy under existing and forthcoming privacy regulations by empowering users to control which websites are authorized to sell their personal information. 


%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/OptOutTime-wild.png}
%	\caption{Distribution of opt outs by COA users as a function of time elapsed  since they first installed the extension.}
%	\label{fig:optdistribution}
%end{figure}

\begin{comment}
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/optsbysite.png}
    \caption{Frequency of opt outs for sites that sell data}
    \label{fig:optfrequency}
\end{figure}
\end{comment}


